Analyzing and Predicting Purchase Intent in E-commerce: Anonymous vs. Identified Customers

The popularity of e-commerce platforms continues to grow. Being able to understand, and predict customer behavior is essential for customizing the user experience through personalized result presentations, recommendations, and special offers. Previous work has considered a broad range of prediction models as well as features inferred from clickstream data to record session characteristics, and features inferred from user data to record customer characteristics. So far, most previous work in the area of purchase prediction has focused on known customers, largely ignoring anonymous sessions, i.e., sessions initiated by a non-logged-in or unrecognized customer. However, in the de-identified data from a large European e-commerce platform available to us, more than 50% of the sessions start as anonymous sessions. In this paper, we focus on purchase prediction for both anonymous and identified sessions on an e-commerce platform. We start with a descriptive analysis of purchase vs. non-purchase sessions. This analysis informs the definition of a feature-based model for purchase prediction for anonymous sessions and identified sessions; our models consider a range of session-based features for anonymous sessions, such as the channel type, the number of visited pages, and the device type. For identified user sessions, our analysis points to customer history data as a valuable discriminator between purchase and non-purchase sessions. Based on our analysis, we build two types of predictors: (1) a predictor for anonymous that beats a production-ready predictor by over 17.54% F1; and (2) a predictor for identified customers that uses session data as well as customer history and achieves an F1 of 96.20%. Finally, we discuss the broader practical implications of our findings.

==> sections/05-modeling_purchase_intent.tex <==
% !TEX root = ../main.tex

\section{Modeling Purchase Intent}
\label{sec:modelingpurchaseintent}

% setting
Next, we use our insights from the previous section to boost purchase intent prediction performance. Since our initial analysis demonstrated that about 56\% of all sessions are anonymous (see Table~\ref{tab:ds_stats}), it is worth to pay special attention to this category. 
Thus, we analyze model performance in two settings: when a user is anonymous (the anonymous setting) and when a user is logged in (the identified setting).

% feature set
Based on the findings obtained thus far and on an analysis of best-performing features available in the literature \citep{hop2013web, lee2015online, niu2017predictive, seippel-2018-customer}, we compile a feature set presented in the Table~\ref{tab:feature_set}. Initially, we added information about previous device type and conversion rate, but we subsequently excluded it from the set because the features decreased classifier performance.
% session data (anon) vs customer history (anon+logged in)
We categorize features into two classes: session features and customer history features. We derive session features from the information of the given session and base customer history features on the information from previous sessions of the given customer.

% anon vs logged features sets
Since we run experiments in anonymous and identified setting, we use different feature set for each setting. For anonymous setting, when a customer is not known, the information about the customer is not available and, therefore, we can only use session features. On the other hand, when a customer is identified, we can use both session and customer history features.
% dynamic vs static
The feature set contains both static and dynamic features. Dynamic features can change throughout the session, whereas static features remain constant.

% our models
After reviewing previous work in the domain of purchase prediction (see Section~\ref{sec:relatedwork}), we choose several models for our experiments: logistic regression, K-nearest neighbors, support vector machines, neural classifier, gradient boosting decision tree, and random forest.

\begin{table}[!h]
\caption{Complete feature set. ``Dynamic'' indicates that a feature may change during a session.}
\label{tab:feature_set}
\begin{tabular}{llcc}
\toprule
\multicolumn{2}{l}{\bf Feature} & \bf Dynamic  & \bf Baseline  \\ 
\midrule
\multirow{8}{*}[-0.1cm]{\rotatebox{90}{Session}}
 & current page dwell time, mean & \checkmark & \checkmark\\
 & current page dwell time, $\sigma$ & \checkmark & \checkmark \\
 & page sequence score & \checkmark & \checkmark \\
 & number of pages & \checkmark & \checkmark\\
 & channel type \\
 & start hour \\
 & week day \\
 & device type \\
 & device conversion rate \\
\midrule
\multirow{9}{*}[0.5cm]{\rotatebox{90}{History}}
 & number of orders  &  & \checkmark \\
 & days since last purchase &  & \checkmark \\
 & number of sessions \\
 & number of devices \\
 & device sequence score \\
 & switch probability \\
\bottomrule
\end{tabular}
\end{table}



==> sections/05-predicting_purchase.tex <==
% !TEX root = ../main.tex

\section{Predicting Purchase}
\label{sec:5}

In this section, we formally describe our prediction task and outline the features used for prediction.





% task
For a given session, we predict whether a user is going to buy or not. We do prediction at several session steps. We define step as number of pages customer seen during session.

% setting
We conduct experiments in two settings. In the first setting, we assume that users are anonymous.
In the second setting, we assume that users are logged in.

% baseline
For a baseline, we use a model currently being deployed in the e-commerce website.

% our model
After reviewing models available for the task, we choose random forest as model for our experiments. We choose this model because of the transparency feature importance of tree-based models. 

% feature set
We analyzed features used in the literature and selected best performing features. The complete feature set is presented in the Table~\ref{tab:feature_set}.


\begin{table}[!htb]
\caption{Complete feature set. An asterisk * indicates that feature changes throughout the session.}
\label{tab:feature_set}
\begin{tabular}{ll}
\hline
\bf Type                           & \bf Feature                                             \\ \hline
\multirow{8}{*}{Session Data}   & current page score* \\
                               					& current page dwell time, mean* \\
                               					& current page dwell time, $\sigma$* \\
                               					& number of pages* \\
                               					& channel type \\
                               					& start hour \\
                               					& week day \\
                               					& device type \\
                               					& device conversion rate \\
\addlinespace
\multirow{8}{*}{Customer History} & number of orders  \\
                               								& days since last purchase  \\
                               								& number of sessions \\
                               								& number of devices \\
                               								& device sequence score \\
                               								& switch probability \\
                               								& previous device type \\
                               								& previous device conversion rate \\ \hline
\end{tabular}
\end{table}

\begin{itemize}
	\item Task definition: given a visit or a customer journey, predict whether the user will end up buying or not.
 	\item data preparation process
\end{itemize}


\begin{figure}[]
\includegraphics[width=0.8\linewidth]{device_feature_importances_per_step_anonymous_setting}
\caption{Relative feature importances across session. End is the last page of the session minus buffer.}
\label{fig:device_feature_importances}
\end{figure}


\subsection{Experimental Setup}

\begin{itemize}
	\item model description: Random Forest with several features
	\item anonymous setting description
	\item logged-in users description
\end{itemize}

\subsection{Results}

\begin{itemize}
	\item results table
	\item results interpretation
	\item Error pattern analysis
\end{itemize}

==> sections/09-conclusions.tex <==
% !TEX root = ../main.tex

\section{Conclusions}
\label{sec:conclusions}

% summary
We explored the

To achieve this, a future research direction would be to not just model but also predict cross-device behaviour. 






==> sections/definitions.tex <==
% !TEX root = ../main.tex

\section{Definitions}
\label{sec:definitions}

% introduction
In the study, we operate with the following definitions:

\begin{description}
% visit
\item[Session] is a sequence of requests made by a single-end user during a visit to a particular site. Session ends if user is idle for more than 30 minutes.
We define two types of sessions: purchase and non-purchase session. Purchase session is a session during which customer buys something. Non-purchase session is a session during which customer does not buy anything.

\item[Session length] is a number of actions taken during given session.

\item[Step] is a number of pages customer seen during given session.

\item[Actions] include opening a new web page, submitting a search query.

% device switch
\item[Device switch] is the act of changing device type in-between sessions.

\item[Moving average]

\item[Moving standard deviation]

\item[Markov Score]

% conversion rate
\item[Conversion rate] is a fraction of the number of visits during which a purchase was made~\cite{moe2004dynamic}. We use this metric to compare device popularity in a purchasing context. The conversion rate can be calculated as follows:
\begin{equation}
\text{\em Conversion rate} = \frac{\text{\em\#purchase\ sessions}}{\text{\em\#all\ sessions}}
\end{equation}

\item[Standardized conversion rate] is used to protect sensitive information. We present standardized conversion rates for each device; since we are interested in differences across devices types, this suffices for our purposes. The \emph{standardized conversation rate} is computed as follows:

\begin{equation}
\begin{split}
\text{\em Standardized}&\text{\em\ conversion rate} = \\
& \frac{\text{\em Conversion rate} - \overline{\text{\em Conversion rate}}}{\sigma}
\end{split}
\end{equation}
where:
\begin{itemize}
	\item $\overline{\text{\em Conversion rate}}$ is the mean conversion rate per device type
	\item $\sigma$ is standard deviation of device-specific conversion rates
\end{itemize}
\end{description}


==> tmp/03-purchase_vs_exploration.tex <==
% !TEX root = ../main.tex

\section{Dataset Description}
\label{sec:3}
\todo{Due: Dec 6}

We start off by distinguishing two search schemes and explaining how we define each of the two. Afterwards, we describe how exploratory and purchasing sessions were mined from the search logs and summarize dataset statistics.

\subsection{Definitions}

This sections describes all the definitions related to the dataset.

% visit
Visit is a 

% conversion rate
Conversion rate is a fraction of visits during which purchase was made (CITE). It can be calculated as follows: TBA

\begin{equation}
Conversion\ rate = \frac{purchase\ visits}{all\ visits}
\end{equation}

% customer journey
Customer journey

% visit distance
We define \textit{distance} between two consecutive sessions $s_t$ and $s_{t+1}$ as the time difference between the last action in the session $s_t$ and the first action of session $s_{t+1}$.




\subsection{Dataset Sampling}

This section explains how dataset was sampled and preprocessed.

% talk about ds sampling


\subsection{Dataset Statistics}

This section describes general dataset statistics and 

The dataset statistics is present in the Table~\ref{tab:ds_stats}.


% finding: purchase visits are longer
From the Table~\ref{tab:ds_stats}, it is clear that an average length of the visits in terms of actions is about six times longer for the sessions where users completed purchase as opposed to the visits where users did not purchase anything.

\begin{table}[!htb]
  \caption{Dataset statistics.}
  \label{tab:ds_stats}
  \begin{tabular}{lrrr}
    \toprule
    Description & Purchase & Non-purchase & Total \\
    \midrule
    Data size, GB		& \numprint{74.12} 		& \numprint{80.8} 			& \numprint{0} \\
    Sessions			& \numprint{3531267} 	& \numprint{27719626}  	& \numprint{0} \\
    Visits          		& \numprint{3649993} 	& \numprint{38055183}  	&  \numprint{0} \\
    \addlinespace
   Rows & \numprint{175725615} & \numprint{234326049} & \\
    Avg. visit length & \numprint{48.14} & \numprint{6.16} & \\
    Customers                             & \numprint{0} & \numprint{0} & \\
   TBA                         & \numprint{0} & \numprint{0} & \\
  \bottomrule
  \end{tabular}
\end{table}

As can be seen form the Table~\ref{tab:ds_device}, the most popular device types are phone and desktop. Interestingly, most purchase visits are from desktop, whereas for most non-purchase visits, phone is  prevailed over desktop by $\approx 1\%$.



\begin{figure}
\includegraphics[width=\linewidth]{purchase_visit_frequency_per_user}
\caption{How many purchasing visits one customer had. The plot demonstrates that about 72\% of customers had only 1 purchasing visit, 28\% - more than one.}
\label{fig:purchase_visit_freq}
\end{figure}


\begin{table}[!htb]
\caption{Dataset characteristics from the device perspective.}
\label{tab:ds_device}
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{Device} & \multicolumn{2}{c}{Purchase visits} & \multicolumn{2}{c}{Non-purchase visits} \\
\cmidrule(r){2-3}\cmidrule{4-5}
       &      size, gb     &     percentage     &      size, gb     &     percentage											\\
\midrule
Phone        	 			&  \numprint{29.85}         		&    40.28    		&  37.55 							& 46.48 	\\
Desktop                  	& 38.40 								&    51.81      		& 36.56 							& 45.25  	 \\
Tablet                  		& 5.86 									&   7.91				& 6.68    							&  8.27 			\\
Game Console           & $4.49 \times 10^{-3}$ 		&  $\approx 0$ 	&  $6.43 \times 10^{-3}$  	&  $\approx 0$ \\
TV                  			& $9.11 \times 10^{-4}$		 	&   $\approx 0$	&  $1.86 \times 10^{-3}$ 	&  $\approx 0$ \\
\addlinespace
Total                  			&  74.11									&    100  			&   80.79							&   100  \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}[!htb]
\caption{User device statistics. \todo{Should I make it bar chart with two variables? It leaves out some data, but shows a clear pattern}}
\label{tab:ds_user_device}
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{Device(s)} & \multicolumn{2}{c}{Purchasers} & \multicolumn{2}{c}{Non-purchasers} \\
\cmidrule(r){2-3}\cmidrule{4-5}
       &      users     &     percentage     &      users     &     percentage											\\
\midrule
Any Device        	 			&  \numprint{2575877}         		&    100    		&  \numprint{5795495} 							& 100 	\\
> 1 device       	& \numprint{173965} & 6.75 & \numprint{1330202} & 22.95  	 \\
\addlinespace
1 device   & \numprint{2401912} &   93.25	& \numprint{4465293} &  77.05 \\
2 devices  & \numprint{169611}	&  6.58 &   \numprint{1232975} & 21.27 \\
3 devices & \numprint{4353}	&  0.17 &   \numprint{97172} & 1.68 \\
4 devices  & \numprint{1}	& $\approx 0$ &   \numprint{55} & $\approx 0$ \\
5 devices & \numprint{0}	&  0 &  0 & 0 \\
\bottomrule
\end{tabular}
\end{table}

%  bar chart, temporarily disabled
\begin{comment}
\begin{figure}
\includegraphics[width=\linewidth]{user_device_chart}
\caption{Fraction of users who own 1,  2, 3, 4, 5 devices. Temporary chart.}
\label{fig:user_device}
\end{figure}
\end{comment}

Table~\ref{tab:ds_user_device} shows that majority of users from both groups use only one device. What is more a bigger fraction of purchasers stick to one device when compared to non-purchasers. In case with two- and three-device users, the situation is opposite: non-purchasers fraction if bigger.


% device ~ purchase visit: where (on which device) users end up buying? 
We would like to know what kind of devices users end up buying with. We count purchasing visits per device and compare counts with non-purchasing visits. The answer is present in the Table~\ref{tab:ds_device_purchase}. As can be seen, the most popular device for purchases is mobile phone, however, desktop has highest conversion rate.


\begin{table}[!htb]
\caption{Purchase visit counts across devices.}
\label{tab:ds_device_purchase}
\begin{tabular}{l rr rr r}
\toprule
\multirow{2}{*}{Device} & \multicolumn{2}{c}{Purchase visits} & \multicolumn{2}{c}{Non-purchase visits} & \multirow{2}{*}{Conv. rate} \\
\cmidrule(r){2-3}\cmidrule{4-5}
       &      visits     &     percentage     &      visits     &     percentage											\\
\midrule
Phone        	 			&  \numprint{1716976}         		&    47.00    		&   \numprint{22121333} 					& 58.09 	& 7.20 \\
Desktop                  	& \numprint{1642820} 			&    44.97      		&  \numprint{13102228} 							& 34.40 & 11.14	 \\
Tablet                  		&  \numprint{293463} 									&   8.03				&  \numprint{2855728}     							&  7.50 	& 	9.32	\\
Game Console           &  \numprint{145} 		&  $\approx 0$ 	&  \numprint{1788}  	&  $\approx 0$ & 7.50 \\
TV                  			&  \numprint{44} 	 	&   $\approx 0$	&   \numprint{695} 	&  $\approx 0$ & 5.95 \\
\addlinespace
Total                  			&   \numprint{3653448} 								&    100  			&    \numprint{38081772} 							&   100  & 8.75 \\
\bottomrule
\end{tabular}
\end{table}





==> tmp/04-dataset_description.tex <==
% !TEX root = ../main.tex

\section{Dataset Description}
\label{sec:3}

We start by distinguishing two search schemes and explaining how we define each of the two. Afterward, we describe how exploratory and purchasing sessions were mined from the search logs and summarize dataset statistics.

\subsection{Definitions}
\label{subsec:definitions}

% introduction
The data set we use comprises 4 weeks of sessions sampled from a European e-commerce website. In the study, we operate with the following definitions:

\begin{description}
% visit
\item[Session] is a sequence of requests made by a single-end user during a visit to a particular site. Session ends if user is idle for more than 30 minutes.
We define two types of sessions: purchase and non-purchase session. Purchase session is a session during which customer buys something. Non-purchase session is a session during which customer does not buy anything.

\item[Session length] is a number of actions taken during given session.

\item[Step] is a number of pages customer seen during given session.

\item[Actions] include opening a new web page, submitting a search query.

% device switch
\item[Device switch] is the act of changing device type in-between sessions.

\item[Moving average]

\item[Moving standard deviation]

\item[Markov Score]

% conversion rate
\item[Conversion rate] is a fraction of the number of visits during which a purchase was made~\cite{moe2004dynamic}. We use this metric to compare device popularity in a purchasing context. The conversion rate can be calculated as follows:
\begin{equation}
\text{\em Conversion rate} = \frac{\text{\em\#purchase\ sessions}}{\text{\em\#all\ sessions}}
\end{equation}

\item[Standardized conversion rate] is used to protect sensitive information. We present standardized conversion rates for each device; since we are interested in differences across devices types, this suffices for our purposes. The \emph{standardized conversation rate} is computed as follows:

\begin{equation}
\begin{split}
\text{\em Standardized}&\text{\em\ conversion rate} = \\
& \frac{\text{\em Conversion rate} - \overline{\text{\em Conversion rate}}}{\sigma}
\end{split}
\end{equation}
where:
\begin{itemize}
	\item $\overline{\text{\em Conversion rate}}$ is the mean conversion rate per device type
	\item $\sigma$ is standard deviation of device-specific conversion rates
\end{itemize}
\end{description}


\subsection{Dataset Sampling}
The data set we use comprises 4 weeks (28 days) of anonymized visits sampled from a European e-commerce website for October 2019. 
Log entries include a unique customer identifier, the class of device the customer used during the session, a timestamp for every query and a URL of each clicked page. 
Besides, we also keep track of the price of every product the customer has seen and the price of the item(s) he or she ended up buying.
In cases where a customer starts a session without logging in and ends up logging in at a later point in the session, we assign the session to the customer.

To filter out bots traffic, we apply several measures related to device type, location, and visit length. First, we specify a set of particular device types we are looking for and remove all the entries from different devices. Moreover, we filter out based on location, including only entries from the European countries from which the majority of the customers come from. 
Besides, we specify visit length, which allows us to get rid of both very short, uninformative visits and abnormally long visits of crawlers~\citep{bomhardt-2005-web}.

\subsection{Dataset Statistics}

TBA


\begin{table}[!htb]
  \caption{Dataset statistics.}
  \label{tab:ds_stats}
  \begin{tabular}{ll}
    \toprule
    \bf Description &  \bf Total \\
    \midrule
    Sessions (total)		&  \numprint{95757177} \\
    Sessions (logged-in customers)                  &  \numprint{41705176} \\
    Sessions (anonymous customers)                  &  \numprint{54144152} \\
    Identified customers         & \numprint{9663509} \\
    Queries	& \numprint{42927} \\
    Devices				& PC, Smartphone, Tablet, Game Console, TV \\
  \bottomrule
  \end{tabular}
\end{table}



==> tmp/tables.tex <==
% !TEX root = ../main.tex

\section{Tmp data}
\todo{Due: Dec 26}

\begin{table}[!htb]
\caption{Dataset characteristic from device perspective.}
\label{tab:ds_device}
\begin{tabular}{lrrrr}
\toprule
\multirow{2}{*}{Device} & \multicolumn{2}{r}{Purchases visits} & \multicolumn{2}{r}{}Non-purchase visits \\
       &      size, gb     &     percentage     &      size, gb     &     percentage											\\
\midrule
Phone        	 			&  \numprint{29.85}         		&    40.28    		&  37.55 							& 46.48 	\\
Desktop                  	& 38.40 								&    51.81      		& 36.56 							& 45.25  	 \\
Tablet                  		& 5.86 									&   7.91				& 6.68    							&  8.27 			\\
Game Console           & $4.49 \times 10^{-3}$ 		&  $\approx 0$ 	&  $6.43 \times 10^{-3}$  	&  $\approx 0$ \\
TV                  			& $9.11 \times 10^{-4}$		 	&   $\approx 0$	&  $1.86 \times 10^{-3}$ 	&  $\approx 0$ \\
\addlinespace
Total                  			&  74.11									&    100  			&   80.79							&   100  \\
\bottomrule
\end{tabular}
\end{table}


